Hypersolvers: Toward Fast Continuous-Depth Models

The infinite-depth paradigm pioneered by Neural ODEs has launched a renaissance in the search for novel dynamical system-inspired deep learning primitives; however, their utilization in problems of non-trivial size has often proved impossible due to poor computational scalability. This work paves the way for scalable Neural ODEs with time-to-prediction comparable to traditional discrete networks. We introduce hypersolvers, neural networks designed to solve ODEs with low overhead and theoretical guarantees on accuracy. The synergistic combination of hypersolvers and Neural ODEs allows for cheap inference and unlocks a new frontier for practical application of continuous-depth models. Experimental evaluations on standard benchmarks, such as sampling for continuous normalizing flows, reveal consistent pareto efficiency over classical numerical methods.

==> app_biblio.tex <==
% standard neural ODE refs
@inproceedings{chen2018neural,
  title={Neural ordinary differential equations},
  author={Chen, Tian Qi and Rubanova, Yulia and Bettencourt, Jesse and Duvenaud, David K},
  booktitle={Advances in neural information processing systems},
  pages={6571--6583},
  year={2018}
}

@article{grathwohl2018ffjord,
  title={Ffjord: Free-form continuous dynamics for scalable reversible generative models},
  author={Grathwohl, Will and Chen, Ricky TQ and Bettencourt, Jesse and Sutskever, Ilya and Duvenaud, David},
  journal={arXiv preprint arXiv:1810.01367},
  year={2018}
}

@article{behrmann2018invertible,
  title={Invertible residual networks},
  author={Behrmann, Jens and Grathwohl, Will and Chen, Ricky TQ and Duvenaud, David and Jacobsen, J{\"o}rn-Henrik},
  journal={arXiv preprint arXiv:1811.00995},
  year={2018}
}

@inproceedings{rubanova2019latent,
  title={Latent Ordinary Differential Equations for Irregularly-Sampled Time Series},
  author={Rubanova, Yulia and Chen, Tian Qi and Duvenaud, David K},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5321--5331},
  year={2019}
}

@article{massaroli2020dissecting,
  title={Dissecting neural odes},
  author={Massaroli, Stefano and Poli, Michael and Park, Jinkyoo and Yamashita, Atsushi and Asama, Hajime},
  journal={arXiv preprint arXiv:2002.08071},
  year={2020}
}

% variants of neural DE
@inproceedings{jia2019neural,
  title={Neural jump stochastic differential equations},
  author={Jia, Junteng and Benson, Austin R},
  booktitle={Advances in Neural Information Processing Systems},
  pages={9843--9854},
  year={2019}
}

@article{poli2019graph,
  title={Graph Neural Ordinary Differential Equations},
  author={Poli, Michael and Massaroli, Stefano and Park, Junyoung and Yamashita, Atsushi and Asama, Hajime and Park, Jinkyoo},
  journal={arXiv preprint arXiv:1911.07532},
  year={2019}
}

@inproceedings{bai2019deep,
  title={Deep equilibrium models},
  author={Bai, Shaojie and Kolter, J Zico and Koltun, Vladlen},
  booktitle={Advances in Neural Information Processing Systems},
  pages={688--699},
  year={2019}
}


%CNF

@inproceedings{yang2019pointflow,
  title={Pointflow: 3d point cloud generation with continuous normalizing flows},
  author={Yang, Guandao and Huang, Xun and Hao, Zekun and Liu, Ming-Yu and Belongie, Serge and Hariharan, Bharath},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={4541--4550},
  year={2019}
}

%PINN
@article{raissi2019physics,
  title={Physics-informed neural networks: A deep learning framework for solving forward and inverse problems involving nonlinear partial differential equations},
  author={Raissi, Maziar and Perdikaris, Paris and Karniadakis, George E},
  journal={Journal of Computational Physics},
  volume={378},
  pages={686--707},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{greydanus2019hamiltonian,
  title={Hamiltonian neural networks},
  author={Greydanus, Samuel and Dzamba, Misko and Yosinski, Jason},
  booktitle={Advances in Neural Information Processing Systems},
  pages={15353--15363},
  year={2019}
}

@article{cranmer2020lagrangian,
  title={Lagrangian neural networks},
  author={Cranmer, Miles and Greydanus, Sam and Hoyer, Stephan and Battaglia, Peter and Spergel, David and Ho, Shirley},
  journal={arXiv preprint arXiv:2003.04630},
  year={2020}
}

% YE OLDE STUFF
@article{zhang2014comprehensive,
  title={A comprehensive review of stability analysis of continuous-time recurrent neural networks},
  author={Zhang, Huaguang and Wang, Zhanshan and Liu, Derong},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  volume={25},
  number={7},
  pages={1229--1262},
  year={2014},
  publisher={IEEE}
}

@article{breen2019newton,
  title={Newton vs the machine: solving the chaotic three-body problem using deep neural networks},
  author={Breen, Philip G and Foley, Christopher N and Boekholt, Tjarda and Zwart, Simon Portegies},
  journal={arXiv preprint arXiv:1910.07291},
  year={2019}
}

%augmentation - regularization
@article{finlay2020train,
  title={How to train your neural ODE},
  author={Finlay, Chris and Jacobsen, J{\"o}rn-Henrik and Nurbekyan, Levon and Oberman, Adam M},
  journal={arXiv preprint arXiv:2002.02798},
  year={2020}
}

@inproceedings{dupont2019augmented,
  title={Augmented neural odes},
  author={Dupont, Emilien and Doucet, Arnaud and Teh, Yee Whye},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3134--3144},
  year={2019}
}

@article{pontryagin1962mathematical,
  title={The mathematical theory of optimal processes},
  author={Pontryagin, Lev Semenovich and Mishchenko, EF and Boltyanskii, VG and Gamkrelidze, RV},
  year={1962},
  publisher={Wiley},
}

@article{paszke2017automatic,
  title={Automatic differentiation in pytorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  year={2017}
}

@article{massaroli2020stable,
  title={Stable Neural Flows},
  author={Massaroli, Stefano and Poli, Michael and Bin, Michelangelo and Park, Jinkyoo and Yamashita, Atsushi and Asama, Hajime},
  journal={arXiv preprint arXiv:2003.08063},
  year={2020}
}

@article{yildiz2019ode,
  title={{ODE2VAE}: Deep generative second order ODEs with Bayesian neural networks},
  author={Y{\i}ld{\i}z, {\c{C}}a{\u{g}}atay and Heinonen, Markus and L{\"a}hdesm{\"a}ki, Harri},
  journal={arXiv preprint arXiv:1905.10994},
  year={2019}
}

% old related work
@inproceedings{li2007algorithm,
  title={The algorithm of neural networks on the initial value problems in ordinary differential equations},
  author={Li-ying, Xu and Hui, Wen and Zhe-zhao, Zeng},
  booktitle={2007 2nd IEEE Conference on Industrial Electronics and Applications},
  pages={813--816},
  year={2007},
  organization={IEEE}
}

@article{xing2010modeling,
  title={Modeling ship equations of roll motion using neural networks},
  author={Xing, Zhiliang and McCue, Leigh},
  journal={Naval Engineers Journal},
  volume={122},
  number={3},
  pages={49--60},
  year={2010},
  publisher={American Society of Naval Engineers}
}

@article{lagaris1998artificial,
  title={Artificial neural networks for solving ordinary and partial differential equations},
  author={Lagaris, Isaac E and Likas, Aristidis and Fotiadis, Dimitrios I},
  journal={IEEE transactions on neural networks},
  volume={9},
  number={5},
  pages={987--1000},
  year={1998},
  publisher={IEEE}
}

@article{lagaris1997artificial,
  title={Artificial neural network methods in quantum mechanics},
  author={Lagaris, Isaac E and Likas, Aristidis and Fotiadis, Dimitrios I},
  journal={Computer Physics Communications},
  volume={104},
  number={1-3},
  pages={1--14},
  year={1997},
  publisher={Elsevier}
}

@article{fang2020neural,
  title={Neural Network Solution of Single-Delay Differential Equations},
  author={Fang, Jie and Liu, Chenglian and Simos, TE and Famelis, I Th},
  journal={Mediterranean Journal of Mathematics},
  volume={17},
  number={1},
  pages={30},
  year={2020},
  publisher={Springer}
}

@article{li2013nonlinearly,
  title={Nonlinearly activated neural network for solving time-varying complex Sylvester equation},
  author={Li, Shuai and Li, Yangming},
  journal={IEEE transactions on cybernetics},
  volume={44},
  number={8},
  pages={1397--1407},
  year={2013},
  publisher={IEEE}
}

@inproceedings{magill2018neural,
  title={Neural networks trained to solve differential equations learn general representations},
  author={Magill, Martin and Qureshi, Faisal and de Haan, Hendrick},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4071--4081},
  year={2018}
}

@article{piscopo2019solving,
  title={Solving differential equations with neural networks: applied to the calculation of cosmological phase transitions},
  author={Piscopo, Maria Laura and Spannowsky, Michael and Waite, Philip},
  journal={arXiv preprint arXiv:1902.05563},
  year={2019}
}

@article{mall2013comparison,
  title={Comparison of artificial neural network architecture in solving ordinary differential equations},
  author={Mall, Susmita and Chakraverty, Snehashish},
  journal={Advances in Artificial Neural Systems},
  volume={2013},
  year={2013},
  publisher={Hindawi}
}

@INPROCEEDINGS{1028323,
  author={K. {Valasoulis} and D. L. {Fotiadis} and I. E. {Lagaris} and A. {Likas}},
  booktitle={2002 14th International Conference on Digital Signal Processing Proceedings. DSP 2002 (Cat. No.02TH8628)}, 
  title={Solving differential equations with neural networks: implementation on a DSP platform}, 
  year={2002},
  volume={2},
  number={},
  pages={1265-1268 vol.2},}
  
  @article {Han8505,
	author = {Han, Jiequn and Jentzen, Arnulf and E, Weinan},
	title = {Solving high-dimensional partial differential equations using deep learning},
	volume = {115},
	number = {34},
	pages = {8505--8510},
	year = {2018},
	publisher = {National Academy of Sciences},
	issn = {0027-8424},
	journal = {Proceedings of the National Academy of Sciences}
}

@article{filici2008neural,
  title={On a neural approximator to ODEs},
  author={Filici, Cristian},
  journal={IEEE transactions on neural networks},
  volume={19},
  number={3},
  pages={539--543},
  year={2008},
  publisher={IEEE}
}

@article{prince1981high,
  title={High order embedded Runge-Kutta formulae},
  author={Prince, Peter J and Dormand, John R},
  journal={Journal of Computational and Applied Mathematics},
  volume={7},
  number={1},
  pages={67--75},
  year={1981},
  publisher={North-Holland}
}

@book{butcher2016numerical,
  title={Numerical methods for ordinary differential equations},
  author={Butcher, John Charles},
  year={2016},
  publisher={John Wiley \& Sons}
}

@inproceedings{schober2014probabilistic,
  title={Probabilistic ODE solvers with Runge-Kutta means},
  author={Schober, Michael and Duvenaud, David K and Hennig, Philipp},
  booktitle={Advances in neural information processing systems},
  pages={739--747},
  year={2014}
}

@article{lu2017beyond,
  title={Beyond finite layer neural networks: Bridging deep architectures and numerical differential equations},
  author={Lu, Yiping and Zhong, Aoxiao and Li, Quanzheng and Dong, Bin},
  journal={arXiv preprint arXiv:1710.10121},
  year={2017}
}

@inproceedings{hauser2017principles,
  title={Principles of Riemannian geometry in neural networks},
  author={Hauser, Michael and Ray, Asok},
  booktitle={Advances in neural information processing systems},
  pages={2807--2816},
  year={2017}
}

@article{chang2017multi,
  title={Multi-level residual networks from dynamical systems view},
  author={Chang, Bo and Meng, Lili and Haber, Eldad and Tung, Frederick and Begert, David},
  journal={arXiv preprint arXiv:1710.10348},
  year={2017}
}

@inproceedings{sonoda2017double,
  title={Double continuum limit of deep neural networks},
  author={Sonoda, Sho and Murata, Noboru},
  booktitle={ICML Workshop Principled Approaches to Deep Learning},
  year={2017}
}

@article{zhu2018convolutional,
title={Convolutional neural networks combined with runge-kutta methods},
author={Zhu, Mai and Chang, Bo and Fu, Chong},
journal={arXiv preprint arXiv:1802.08831},
year={2018}}

@article{demeester2019system,
  title={System Identification with Time-Aware Neural Sequence Models},
  author={Demeester, Thomas},
  journal={arXiv preprint arXiv:1911.09431},
  year={2019}
}

@article{both2019deepmod,
  title={DeepMoD: Deep learning for Model Discovery in noisy data},
  author={Both, Gert-Jan and Choudhury, Subham and Sens, Pierre and Kusters, Remy},
  journal={arXiv preprint arXiv:1904.09406},
  year={2019}
}

@article{winovich2019convpde,
  title={ConvPDE-UQ: Convolutional neural networks with quantified uncertainty for heterogeneous elliptic partial differential equations on varied domains},
  author={Winovich, Nick and Ramani, Karthik and Lin, Guang},
  journal={Journal of Computational Physics},
  volume={394},
  pages={263--279},
  year={2019},
  publisher={Elsevier}
}

@article{regazzoni2019machine,
  title={Machine learning for fast and reliable solution of time-dependent differential equations},
  author={Regazzoni, Francesco and Dede, Luca and Quarteroni, Alfio},
  journal={Journal of Computational Physics},
  volume={397},
  pages={108852},
  year={2019},
  publisher={Elsevier}
}

@article{long2019pde,
  title={PDE-Net 2.0: Learning PDEs from data with a numeric-symbolic hybrid deep network},
  author={Long, Zichao and Lu, Yiping and Dong, Bin},
  journal={Journal of Computational Physics},
  volume={399},
  pages={108925},
  year={2019},
  publisher={Elsevier}
}

@article{raissi2018deep,
  title={Deep hidden physics models: Deep learning of nonlinear partial differential equations},
  author={Raissi, Maziar},
  journal={The Journal of Machine Learning Research},
  volume={19},
  number={1},
  pages={932--955},
  year={2018},
  publisher={JMLR. org}
}

@article{qin2019data,
  title={Data driven governing equations approximation using deep neural networks},
  author={Qin, Tong and Wu, Kailiang and Xiu, Dongbin},
  journal={Journal of Computational Physics},
  volume={395},
  pages={620--635},
  year={2019},
  publisher={Elsevier}
}

@article{raissi2018multistep,
  title={Multistep neural networks for data-driven discovery of nonlinear dynamical systems},
  author={Raissi, Maziar and Perdikaris, Paris and Karniadakis, George Em},
  journal={arXiv preprint arXiv:1801.01236},
  year={2018}
}

@article{weinan2018deep,
  title={The deep Ritz method: a deep learning-based numerical algorithm for solving variational problems},
  author={Weinan, E and Yu, Bing},
  journal={Communications in Mathematics and Statistics},
  volume={6},
  number={1},
  pages={1--12},
  year={2018},
  publisher={Springer}
}

@article{khoo2019switchnet,
  title={SwitchNet: a neural network model for forward and inverse scattering problems},
  author={Khoo, Yuehaw and Ying, Lexing},
  journal={SIAM Journal on Scientific Computing},
  volume={41},
  number={5},
  pages={A3182--A3201},
  year={2019},
  publisher={SIAM}
}

@article{parisi2019continual,
  title={Continual lifelong learning with neural networks: A review},
  author={Parisi, German I and Kemker, Ronald and Part, Jose L and Kanan, Christopher and Wermter, Stefan},
  journal={Neural Networks},
  year={2019},
  publisher={Elsevier}
}

@article{howard2018universal,
  title={Universal language model fine-tuning for text classification},
  author={Howard, Jeremy and Ruder, Sebastian},
  journal={arXiv preprint arXiv:1801.06146},
  year={2018}
}

@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@article{ganin2016domain,
  title={Domain-adversarial training of neural networks},
  author={Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
  journal={The Journal of Machine Learning Research},
  volume={17},
  number={1},
  pages={2096--2030},
  year={2016},
  publisher={JMLR. org}
}

@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle={Advances in neural information processing systems},
  pages={2672--2680},
  year={2014}
}

@article{kidger2020neural,
  title={Neural Controlled Differential Equations for Irregular Time Series},
  author={Kidger, Patrick and Morrill, James and Foster, James and Lyons, Terry},
  journal={arXiv preprint arXiv:2005.08926},
  year={2020}
}

@book{hester2013texplore,
  title={TEXPLORE: Temporal Difference Reinforcement Learning for Robots and Time-Constrained Domains},
  author={Hester, Todd},
  publisher={Springer},
    year={2013}
}

@article{runge1895numerische,
  title={{\"U}ber die numerische Aufl{\"o}sung von Differentialgleichungen},
  author={Runge, Carl},
  journal={Mathematische Annalen},
  volume={46},
  number={2},
  pages={167--178},
  year={1895},
  publisher={Springer}
}

@inproceedings{james2019sim,
  title={Sim-to-real via sim-to-sim: Data-efficient robotic grasping via randomized-to-canonical adaptation networks},
  author={James, Stephen and Wohlhart, Paul and Kalakrishnan, Mrinal and Kalashnikov, Dmitry and Irpan, Alex and Ibarz, Julian and Levine, Sergey and Hadsell, Raia and Bousmalis, Konstantinos},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={12627--12637},
  year={2019}
}

@inproceedings{gupta2018meta,
  title={Meta-reinforcement learning of structured exploration strategies},
  author={Gupta, Abhishek and Mendonca, Russell and Liu, YuXuan and Abbeel, Pieter and Levine, Sergey},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5302--5311},
  year={2018}
}

@book{shampine2018numerical,
  title={Numerical solution of ordinary differential equations},
  author={Shampine, Lawrence F},
  year={2018},
  publisher={Routledge}
}

@article{dormand1980family,
  title={A family of embedded Runge-Kutta formulae},
  author={Dormand, John R and Prince, Peter J},
  journal={Journal of computational and applied mathematics},
  volume={6},
  number={1},
  pages={19--26},
  year={1980},
  publisher={Elsevier}
}

@article{loshchilov2017decoupled,
  title={Decoupled weight decay regularization},
  author={Loshchilov, Ilya and Hutter, Frank},
  journal={arXiv preprint arXiv:1711.05101},
  year={2017}
}

@inproceedings{he2015delving,
  title={Delving deep into rectifiers: Surpassing human-level performance on imagenet classification},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1026--1034},
  year={2015}
}

@article{kobyzev2019normalizing,
  title={Normalizing flows: Introduction and ideas},
  author={Kobyzev, Ivan and Prince, Simon and Brubaker, Marcus A},
  journal={arXiv preprint arXiv:1908.09257},
  year={2019}
}

@article{cash2003efficient,
  title={Efficient numerical methods for the solution of stiff initial-value problems and differential algebraic equations},
  author={Cash, JR},
  journal={Proceedings of the Royal Society of London. Series A: Mathematical, Physical and Engineering Sciences},
  volume={459},
  number={2032},
  pages={797--815},
  year={2003},
  publisher={The Royal Society}
}

@article{shampine1979user,
  title={A user’s view of solving stiff ordinary differential equations},
  author={Shampine, Lawrence F and Gear, Charles William},
  journal={SIAM review},
  volume={21},
  number={1},
  pages={1--17},
  year={1979},
  publisher={SIAM}
}

@article{mclachlan1998numerical,
  title={Numerical integrators that preserve symmetries and reversing symmetries},
  author={McLachlan, Robert I and Quispel, GRW and Turner, Grant Stephen},
  journal={SIAM journal on numerical analysis},
  volume={35},
  number={2},
  pages={586--599},
  year={1998},
  publisher={SIAM}
}

@article{hernandez2018time,
  title={Time-symmetric integration in astrophysics},
  author={Hernandez, David M and Bertschinger, Edmund},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={475},
  number={4},
  pages={5570--5584},
  year={2018},
  publisher={Oxford University Press}
}

==> commons.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{mathtools}
\usepackage[bb=boondox,bbscaled=.95]{mathalfa}
\usepackage{hyperref}
\usepackage{bm}
\usepackage{cancel}
\usepackage{thmtools, thm-restate}
\usepackage{wrapfig}
% plotting
\usepackage{pgfplots}
\usepackage{tikz}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{patchplots}
\pgfplotsset{compat=1.16} 

%% THEOREMS
\declaretheorem{theorem}
\newtheorem{lemma}{Lemma}

\newtheorem{defn}{Definition}
\newtheorem{rmk}{Remark}
\newtheorem{note}{Note}
\newtheorem{proposition}[defn]{Proposition}
\newtheorem{example}[defn]{Example}

% BBs
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\A}{\mathbb{A}}

% Cals
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cT}{\mathcal{T}}

\newcommand{\nx}{{n_x}}
\newcommand{\nz}{{n_z}}
\newcommand{\ny}{{n_y}}
\newcommand{\nt}{{n_\theta}}
\newcommand{\nw}{{n_\omega}}
\newcommand{\x}{\times}
\newcommand{\ra}{\rightarrow}
\newcommand{\eps}{\epsilon}

\newcommand{\z}{\mathbf{z}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cb}{\mathbf{c}}

\def\red{\color{red}}
\def\lblue{\color{blue!50!white}}
\definecolor{flow}{rgb}{0.5686274509803921, 0.5764705882352941, 0.7294117647058823}

\newcommand{\fcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0.03) circle ;}

% LaTeX code
\usepackage{minted}



